A Sum-of-Ratios Multi-Dimensional-Knapsack Decomposition for DNN Resource Scheduling

In recent years, to sustain the resource-intensive computational needs for training deep neural networks (DNNs), it is widely accepted that exploiting the parallelism in large-scale computing clusters is critical for the efficient deployments of DNN training jobs. However, existing resource schedulers for traditional computing clusters are not well suited for DNN training, which results in unsatisfactory job completion time performance. The limitations of these resource scheduling schemes motivate us to propose a new computing cluster resource scheduling framework that is able to leverage the special layered structure of DNN jobs and significantly improve their job completion times. Our contributions in this paper are three-fold: i) We develop a new resource scheduling analytical model by considering DNN's layered structure, which enables us to analytically formulate the resource scheduling optimization problem for DNN training in computing clusters; ii) Based on the proposed performance analytical model, we then develop an efficient resource scheduling algorithm based on the widely adopted parameter-server architecture using a sum-of-ratios multi-dimensional-knapsack decomposition (SMD) method to offer strong performance guarantee; iii) We conduct extensive numerical experiments to demonstrate the effectiveness of the proposed schedule algorithm and its superior performance over the state of the art.

==> Appdx_A/Appdx_A.tex <==
% !TEX root = ../ML_Networking_INFOCOM20.tex

\section{Proof of Lemma~\ref{lemma:wait}}\label{appdx:lem_wait}
% To overcome the major limitation of the sequential based model (i.e., no parameter synchronization is considered), this model utilizes the overlap between the BP and the communication.
Note that the wait-free model  performs communication at layer level.
For example, as shown in Fig.~\ref{fig:waitfree}, the last layer $L_4$ starts sending gradients once its BP finishes.
Likewise, $L_3$ can immediately start sending after $L_4$ completes it since $L_3$ already finishes BP at that time.
Receiving parameters of $L_4$ and sending gradients of $L_3$ can be done concurrently if full-duplex communication is allowed.
However, $L_3$ needs to wait for the completion of $L_4$ receiving parameters before starting to receive.
The analysis of other layers also follows similarly.

We can extend our analysis to the general case.
The last layer $L_N$ can immediately start sending gradients once it finishes BP, i.e., $\kappa_N=b_N$.
The BP is conducted continuously in the reverse layer order, thus $\sum_{k=j}^Nb_k$ is the time when layer $j$ finishes BP.
The layer $j +   1$ starts sending gradients at time $\kappa_{j+1}$ and it takes $r_{j+1}$ time to finish.
Hence, layer $j +   1$ can finish sending at time $\kappa_{j+1} +   r_{j+1}$.
Note that layer $j \neq    N$ can not start sending gradients until this layer finishes BP and its following layer $j +   1$ completes sending gradients since that layer can not be preempted once it gets started.
Hence, the start time of sending gradients is 
% the maximum between these two times, i.e.,
$\kappa_j=\max\{\sum_{k=j}^Nb_k,\kappa_{j+1}+r_{j+1}\}$, which proves Eqn.~(\ref{wait_free_kappa}).

Next we consider the time when layer $j$ starts receiving parameters.
The layer $L_N$ can immediately start receiving once it finishes sending gradients, i.e., $s_N=b_N +   r_N$.
The layer $j$ starts sending gradients at $\kappa_j$ and it takes $r_j$ time to do sending.
Thus it completes sending at time $\kappa_j +   r_j$.
The layer $j +   1$ starts receiving at time $s_{j+1}$ and takes $r_{j+1}$ to do the receiving.
Thus, it completes receiving parameters at time $s_{j+1} +   r_{j+1}$.
For layers $j \neq    N$, layer $j$ cannot start receiving parameters until this layer completes sending gradients and its subsequent layer $j +   1$ finishes receiving parameters.
Hence, the start time of receiving parameters is 
% the maximum between these two times, i.e.,
$s_j=\max\{\kappa_j+r_j,s_{j+1}+r_{j+1}\}$, which proves Eqn.~(\ref{wait_free_s}).
% Take Fig.~\ref{fig:waitfree} as an example, $L_3$ starts sending gradients after it finishes BP and its subsequent layer $L_4$ finishes sending gradients.
% And $L_3$ starts receiving parameters as soon as it finishes sending gradients and its subsequent layer $L_4$ completes receiving parameters.

Lastly we analyze the start time of FP at layer $j$.
The first layer $L_1$ can start FP immediately after it finishes receiving parameters, i.e., $\tau_i=s_1+r_1$.
The layer $j \neq    1$ can only start FP on the condition that both its previous layer $j -   1$ finishes FP and this layer finishes receiving parameters.
% i.e., $\tau_j=\max\{t_j+r_j,\tau_{j-1}+f_{j-1}\}$.
% However, this model ensures that the last layer finishes the communication first, followed by the penultimate layer, and the initial layer is the last one to complete the communication.
However, the wait-free model ensures that the communication is finished in the reverse layer order, thus the FP is processed continuously, i.e., the layer $j$ can start FP immediately once the layer $j -   1$ finishes.
% Thus this layer can start FP as long as its previous layer finishes it.
Hence, the start time of FP at layer $j$ is $\tau_j= \tau_{j-1}+f_{j-1}$, which proves Eqn.~(\ref{wait_free_tau}).
Lastly, we can have the training time for an iteration $t=\tau_N+f_N$.
This completes the proof.
% where $\tau_N$ can be replaced by Eqn.~(\ref{wait_free_tau}).

% Take the Fig.~\ref{fig:waitfree}(b) as an example, we can compute $t$ as follows:
% \begin{align}
%     t=&\underbrace{b_4}_{H_b}+\underbrace{2r_4+r_3+r_2+r_1}_{H_r}+\underbrace{\sum_{j=1}^4f_j}_{H_f}.
% \end{align}


==> Appdx_B/Appdx_B.tex <==
% !TEX root = ../ML_Networking_INFOCOM20.tex

%\section{Proof Sketch of Theorem~\ref{thm_Competitive}} \label{appdx:thm_Competitive}

\section{Proof of Lemma~\ref{lemma:priority}} \label{appdx:lem_priority}
% The major limitation of wait free based model is that the communication channel is idle in FP. 
% The priority based model further to utilize the overlap between the communication and computation by assigning the priority to each layer based on when its data will be used in the next iteration.
%Fig.~\ref{fig:priority}(c) illustrates the model, 
% where it assigns the highest priority to the first layer and the lowest priority to the last layer 
% % since it can proceed to the next iteration as long as the initial layer finishes receiving parameters.
% based on when the data will be used in the next iteration.
% We consider the model that allows preemption (i.e. the higher priority layer can  preempt the lower priority layer) and parameter slicing, which is the state of the art.
% Parameter slicing is instead of transfer the full parameters of each layer, we slice them into smaller unit size $\nu$, which is the greatest common divisor of communication and computation time among all layers.
% And as a result, the layers can be roughly aligned since each layer is divisible by $\nu$.
% The communication time then will be reduced significantly as demonstrated in Fig.~\ref{fig:slicing}, where it can approach to half of the total communication time as the dashed line indicates.
% If no preemption occurred at layer $j$, We can project sliced parameters as the dashed line shows in Fig.~\ref{fig:slicing}, and then the communication time of layer $j$ can be estimated as $r_j +   u$.
% The total communication time of layer $j$ depends on whether it is preempted.

The total communication time of a layer $j$ in the priority-based model depends on how many times it is preempted.
However the extra receiving parameters time introduced by the preemption can be done concurrently while its preceding layers' are sending gradients, thus, the preemption has no impact on the communication time.
For example, in Fig.~\ref{fig:priority}, the first slice of receiving parameters of layer $L_4$ can be processed concurrently with the first slice of sending gradients slice of layer $L_3$.

%At first glance, it seems intractable to compute $e_j$ since each layer depends on computation and communication distribution of its previous layers.
Now, we note that the end communication time of layer $j$ does not need to be calculated if it can finish before some of its preceding layers, i.e., no later than at $\max_{1\leq k\leq j-1}\{e_j\}$.
Under this condition, layer $j$ is guaranteed to finish communication when layer $j -   1$ completes FP and it can immediately start FP when layer $j -   1$ finishes, i.e., $\tau_j=\tau_{j-1} +   f_{j-1}$.
Take Fig.~\ref{fig:priority} again as an example, $L_2$ finishes communication no later than $L_1$ finishes, i.e., $e_2 \leq  e_1$.
Hence we do not need to calculate the exact $e_2$ to compute $\tau_2$ because $L_2$ is guaranteed to complete communication when $L_1$ finishes FP, where $\tau_2=e_1+f_1$.
The observation leads to an easier calculation of $\tau_j$, where we only need to compute the exact end communication time when $e_j > \max_{1\leq k\leq j-1}\{e_j\}$; otherwise, we can assign some small number (e.g., 0) to $e_j$.
% otherwise we update the maximum end communication time among $j$ layers.

In the priority-based model, the first layer has the highest priority and can start communication immediately after finishing BP (i.e.,at time $\sum_{k=1}^Nb_k$).
The total communication time is $r_1 +   \nu$.
Thus, the end communication time is
$e_1=\sum_{k=1}^Nb_k +   r_1 +   \nu$.
Next we consider $j \neq    1$, where the key is to calculate its remaining end communication time if it takes the longest time to finish among all its preceding layers.
In this case, it appends the remaining communication time to the maximum end communication time, i.e., $e_{\max}\triangleq\max_{1\leq k\leq j-1}\{e_k\}$.

We observe that if we project each layer's communication time to the first layer, we will have $\nu$ time of sending gradients, $\sum_{k=1}^j r_k$ time of concurrent sending gradients and receiving parameters, and $\nu$ time of receiving parameters.
When we compute the remaining communication time of layer $j$, we need to check whether all $j-1$ layers ($L_2$ to $L_j$) can place their communication into the BP time slots ($L_1$ starts communication after it finishes BP, thus it does not take up the BP slots), i.e., $\sum_{k=2}^jr_k -    \sum_{k=1}^{j-1}b_k$. 
If no, we need to append the remaining communication time to $e_{\max}$.
Hence, we can set $e_j=0$ when $\sum_{k=2}^j r_k\leq \sum_{k=1}^{j-1}b_k$; otherwise, we can set it to $\max_{1\leq k\leq j-1} \{e_k\} +   \sum_{k=2}^jr_k -    \sum_{k=1}^{j-1}b_k$.
This proves Eq.~(\ref{priority_e}).

Lastly, we compute the start time of FP, for which we consider the following two cases:
If layer $j$ can finish communication before some of its preceding layer (i.e., $e_j=0$), then it can start FP immediately after its preceding layer $j -   1$ completes FP.
Thus, $\tau_j=\tau_{j-1} +   f_{j-1}$.
Otherwise, it needs to wait until it finishes communication.
Thus, the start time of FP of layer $j$ is $\tau_j=\max\{\tau_{j-1} +   f_{j-1}, e_j\}$.
We can merge this two conditions as shown in Eqn.~(\ref{priority_tau}).
Finally, the training time for an iteration is $t=\tau_N+f_N$ and the proof is complete.

% Take the Fig.~\ref{fig:priority}(c) as an example, we can compute $t$ as follows:
% \begin{align}
%     t=&\underbrace{b_4+b_3+b_2}_{H_b}+\underbrace{r_2+r_1+\nu}_{H_r}+\underbrace{f_4+f_3+f_2+f_1}_{H_f}.
% \end{align}




==> Appdx_C/Appdx_C.tex <==
% !TEX root = ../ML_Networking_INFOCOM20.tex

\section{Proof of Lemma~\ref{lem_ILP}} \label{appdx:lem_ILP}
To prove Lemma~\ref{lem_ILP}, consider the probabilities of the following ``bad'' events: 1) $\sum_{l=1}^L \frac{\mathbf{a}_l^{\top}\hat{\mathbf{x}}}{\mathbf{d}_l^{\top}\hat{\mathbf{x}}} +   \mathbf{c}^{\top} \hat{\mathbf{x}} >  \frac{8L/M_\delta+4}{\delta}\sum_{l=1}^L (\frac{\mathbf{a}_l^{\top}\bar{\mathbf{x}}}{\mathbf{d}_l^{\top}\bar{\mathbf{x}}}+\mathbf{c}^{\top} \bar{\mathbf{x}})$ ($M_\delta$ will be defined later); and 2) $\exists i$ such that $(\mathbf{B}\hat{\mathbf{x}})_{i} > b_{i}$.
Note that events 2) can be equivalently rewritten as: 2') $\exists i$ such that $\mathbb{E}\{(\mathbf{B}\hat{\mathbf{x}})_{i} \frac{W_{b}}{b_{i}} > W_{b}\}$.
Since $\mathbb{E}\{ \hat{\mathbf{x}} \} =\mathbf{x}'=M_\delta\bar{\mathbf{x}}$, by linearity of expectation, we have:
% \vspace{-.2in}
\begin{align}
\nonumber\label{eqn_exp1}\mathbb{E}\bigg\{\sum_{l=1}^L \frac{\mathbf{a}_l^{\top}\hat{\mathbf{x}}}{\mathbf{d}_l^{\top}\hat{\mathbf{x}}} +   \mathbf{c}^{\top} \hat{\mathbf{x}} \bigg\}
&=\sum_{l=1}^L\mathbb{E}\bigg\{ \frac{\mathbf{a}_l^{\top}\hat{\mathbf{x}}}{\mathbf{d}_l^{\top}\hat{\mathbf{x}}}\bigg\} +   \mathbb{E}\{\mathbf{c}^{\top} \hat{\mathbf{x}}\}\\
&=\sum_{l=1}^L\mathbb{E}\bigg\{ \frac{\mathbf{a}_l^{\top}\hat{\mathbf{x}}}{\mathbf{d}_l^{\top}\hat{\mathbf{x}}}\bigg\}+M_\delta\mathbf{c}^{\top} \bar{\mathbf{x}}, \\
%
% \label{eqn_exp2}& \mathbb{E}\left\{ (\A\hat{\x})_{i} \frac{W_{a}}{a_{i}} \right\} = G \mathbb{E} \left\{ (\A\bar{\x})_{i}\frac{W_{a}}{a_{i}} \right\} \geq GW_{a}, \\
%
\label{eqn_exp3} \mathbb{E}\left\{ (\mathbf{B}\hat{\mathbf{x}})_{i} \frac{W_{b}}{b_{i}} \right\} &= M_\delta\mathbb{E}\{(\mathbf{B}\bar{\mathbf{x}})_{i}\frac{W_{b}}{b_{i}}\} \leq M_\delta W_{b}.
\vspace{-.2in}
\end{align}

We observe that the integer solution obtained from the fractional solution using randomized rounding has a maximum gap of 1, i.e., $\hat{x}_i -   1\leq M_\delta\bar{x}_i\leq \hat{x}_i +   1$, hence we can compute the following expectation:
\begin{align}
\nonumber\label{eqn_obj}\mathbb{E}\left\{\frac{ \frac{\mathbf{a}_l^{\top}\hat{\mathbf{x}}}{\mathbf{d}_l^{\top}\hat{\mathbf{x}}}}{{\frac{\mathbf{a}_l^{\top}\bar{\mathbf{x}}}{\mathbf{d}_l^{\top}\bar{\mathbf{x}}}}} \right \}& \leq  \mathbb{E}\left \{ \frac{\mathbf{a}_l^{\top}(M_\delta\bar{\mathbf{x}}+\mathbf{1})}{\mathbf{a}_l^{\top}\bar{\mathbf{x}}}\cdot\frac{\mathbf{d}_l^{\top}(\hat{\mathbf{x}} +   \mathbf{1})}{M_\delta\mathbf{d}_l^{\top}\hat{\mathbf{x}}}\right \}\\
&\leq\mathbb{E}\left \{ \frac{\mathbf{a}_l^{\top}(\bar{\mathbf{x}}+\mathbf{1})}{\mathbf{a}_l^{\top}\bar{\mathbf{x}}}\cdot\frac{\mathbf{d}_l^{\top}(\hat{\mathbf{x}} +   \mathbf{1})}{M_\delta\mathbf{d}_l^{\top}\hat{\mathbf{x}}}\right \}\nonumber\\
&\overset{(a)}{\leq}\frac{4}{M_\delta},
% \nonumber\label{eqn_obj}\mathbb{E}\left\{\frac{ \frac{\mathbf{a}_l^{\top}\hat{\mathbf{x}}}{\mathbf{d}_l^{\top}\hat{\mathbf{x}}}}{{\frac{\mathbf{a}_l^{\top}\bar{\mathbf{x}}}{\mathbf{d}_l^{\top}\bar{\mathbf{x}}}}} \right \}&=\mathbb{E}\left \{ \frac{\mathbf{a}_l^{\top}\hat{\mathbf{x}}}{\mathbf{a}_l^{\top}\bar{\mathbf{x}}}\cdot\frac{\mathbf{d}_l^{\top}\bar{\mathbf{x}}}{\mathbf{d}_l^{\top}\hat{\mathbf{x}}}\right \}\\
% & \leq  \mathbb{E}\left \{ \frac{\mathbf{a}_l^{\top}(\bar{\mathbf{x}}+\mathbf{1})}{\mathbf{a}_l^{\top}\bar{\mathbf{x}}}\cdot\frac{\mathbf{d}_l^{\top}(\hat{\mathbf{x}} +   \mathbf{1})}{\mathbf{d}_l^{\top}\hat{\mathbf{x}}}\right \} \leq  4
\end{align}
where (a) follows the fact that $\bar{\mathbf{x}},\hat{\mathbf{x}}\geq 1$.

\begin{lem}
\label{lem:relation} Let  $A(\mathbf{x})\!=\!\frac{\sum_{k=1}^nf(k,\mathbf{x})}{\sum_{k=1}^ng(k,\mathbf{x})}$, and $B(\mathbf{x})\!=\!\sum_{k=1}^n\frac{f(k,\mathbf{x})}{g(k,\mathbf{x})}$.
If both $f(\cdot)$ and $g(\cdot)$ are non-negativity, then we have $A(\mathbf{x})\leq B(\mathbf{x})$.
\end{lem}

\begin{proof}
$\frac{f(k,\mathbf{x})}{\sum_{k=1}^ng(k,\mathbf{x})}\leq\frac{f(k,\mathbf{x})}{g(k,\mathbf{x})}$, since $g(k,\mathbf{x})\leq\sum_{k=1}^ng(k,\mathbf{x})$.
Thus $A(\mathbf{x})=\frac{\sum_{k=1}^nf(k,\mathbf{x})}{\sum_{k=1}^ng(k,\mathbf{x})}=\sum_{k=1}^n\frac{f(k,\mathbf{x})}{\sum_{k=1}^ng(k,\mathbf{x})}\leq\sum_{k=1}^n\frac{f(k,\mathbf{x})}{g(k,\mathbf{x})}=B(\mathbf{x})$.
\end{proof}


Then, by Markov inequality (\ref{eqn_exp1}) and (\ref{eqn_obj}), and Lemma~\ref{lem:relation}, we have 
\begin{align*}
&\mathrm{Pr} \left\{ \frac{\sum_{l=1}^L \frac{\mathbf{a}_l^{\top}\hat{\mathbf{x}}}{\mathbf{d}_l^{\top}\hat{\mathbf{x}}}+\mathbf{c}^{\top} \hat{\mathbf{x}}}{\sum_{l=1}^L \frac{\mathbf{a}_l^{\top}\bar{\mathbf{x}}}{\mathbf{d}_l^{\top}\bar{\mathbf{x}}}+\mathbf{c}^{\top} \bar{\mathbf{x}}}> \frac{8L/M_\delta+4}{\delta} \right\}\\
&\leq \frac{\mathbb{E}\left\{\frac{\sum_{l=1}^L \frac{\mathbf{a}_l^{\top}\hat{\mathbf{x}}}{\mathbf{d}_l^{\top}\hat{\mathbf{x}}}+\mathbf{c}^{\top} \hat{\mathbf{x}}}{\sum_{l=1}^L \frac{\mathbf{a}_l^{\top}\bar{\mathbf{x}}}{\mathbf{d}_l^{\top}\bar{\mathbf{x}}}+\mathbf{c}^{\top} \bar{\mathbf{x}}} \right \}}{\frac{8L/M_\delta+4}{\delta}}\leq \frac{\mathbb{E}\left\{\frac{\sum_{l=1}^L \frac{\mathbf{a}_l^{\top}\hat{\mathbf{x}}}{\mathbf{d}_l^{\top}\hat{\mathbf{x}}}}{\sum_{l=1}^L \frac{\mathbf{a}_l^{\top}\bar{\mathbf{x}}}{\mathbf{d}_l^{\top}\bar{\mathbf{x}}}} + \frac{\mathbf{c}^{\top} \hat{\mathbf{x}}}{\mathbf{c}^{\top} \bar{\mathbf{x}}}\right \}}{\frac{8L/M_\delta+4}{\delta}}\\
&\leq \frac{\mathbb{E}\left\{\sum_{l=1}^L\bigg(\frac{ \frac{\mathbf{a}_l^{\top}\hat{\mathbf{x}}}{\mathbf{d}_l^{\top}\hat{\mathbf{x}}}}{ \frac{\mathbf{a}_l^{\top}\bar{\mathbf{x}}}{\mathbf{d}_l^{\top}\bar{\mathbf{x}}}}\bigg ) + \frac{\mathbf{c}^{\top} \hat{\mathbf{x}}}{\mathbf{c}^{\top} \bar{\mathbf{x}}}\right \}}{\frac{8L/M_\delta+4}{\delta}}
\leq \frac{\mathbb{E}\left\{\sum_{l=1}^L\bigg(\frac{ \frac{\mathbf{a}_l^{\top}\hat{\mathbf{x}}}{\mathbf{d}_l^{\top}\hat{\mathbf{x}}}}{ \frac{\mathbf{a}_l^{\top}\bar{\mathbf{x}}}{\mathbf{d}_l^{\top}\bar{\mathbf{x}}}}\bigg ) + \frac{\mathbf{c}^{\top} (M_\delta\bar{\mathbf{x}}+1)}{\mathbf{c}^{\top} \bar{\mathbf{x}}}\right \}}{\frac{8L/M_\delta+4}{\delta}}\\
&\leq \frac{4L/M_\delta+2}{(8L/M_\delta+4)/\delta}=\frac{\delta}{2}.
\end{align*}
%

Next, we note that each $\hat{x}_{j}$ can be viewed as a sum of independent random variables in $[0,1]$ as follows:
The fixed part of $\lfloor x'_j \rfloor$ is a sum of $\lfloor x'_j \rfloor$ random variables with value 1 with probability 1.
Then, we have that $(\mathbf{B}\hat{\mathbf{x}})_{i} \frac{W_b}{b_{i}}= (\sum_{j}[\mathbf{B}]_{ij}\hat{x}_{j}) \frac{W_b}{b_{i}}$ is also a sum of independent random variables in $[0,1]$.
Using Chernoff bound, we have $\mathrm{Pr} \{ (\mathbf{B}\hat{\mathbf{x}})_{i} \frac{W_{b}}{b_{i}} > (1+\epsilon)M_\delta W_{b} \} \leq  \exp( -\epsilon^{2} \frac{M_\delta W_{b}}{3} )$.
Setting $(1+\epsilon)M_\delta=1$, i.e., $\epsilon=\frac{1}{M_\delta} -   1$, we have:
\begin{align}
\mathrm{Pr} \{ (\mathbf{B}\hat{\mathbf{x}})_{i} \frac{W_{b}}{b_{i}} >  W_b\} \leq  \exp(-(\frac{1}{M_\delta} -   1)^2M_\delta\frac{W_b}{3})   
\end{align}
Forcing $\exp(-(\frac{1}{M_\delta} -   1)^2M_\delta\frac{W_b}{3})\triangleq \frac{\delta}{2r}$ and solving $M_\delta$, we have:
\begin{align} \label{eqn_L_def}
M_\delta \triangleq 1 +    \frac{3\ln(2r/\delta)}{2W_b} -     \sqrt{ \bigg(\frac{3\ln(2r/\delta)}{2W_b} \bigg)^{2} +    \frac{3\ln(2r/\delta)}{W_b} }, \!\!\!
\end{align}
which implies that
\begin{align}
\mathrm{Pr} \{ (\mathbf{B}\hat{\mathbf{x}})_{i} \frac{W_{b}}{b_{i}} >  W_b\}\leq\frac{\delta}{2r}.   
\end{align}
Therefore we have that events 1)--2) occur with probability less than $\frac{\delta}{2} + r\cdot\frac{\delta}{2r} = \delta$, and the proof is complete.


==> Sec7_Prelim/Sec7_Prelim.tex <==
% !TEX root = ../ML_Networking_INFOCOM20.tex

\section{Deep Neural Network Training in Computing Clusters: A Primer}
\label{sec:prelim}

Although significant progress of DNNs has been made recently, computing system research on facilitating distributed DNN training remains in its infancy.
In this section, we provide a quick overview on this fast-growing area to familiarize readers with related background and fix the terminologies.

\subsection{Distributed DNN Training}
%As mentioned earlier, since training DNN is time-consuming and resource-intensive, 
Exploiting parallelism in large-scale computing clusters for DNN training has become increasingly important.
In this paper, we focus on data parallelism with the widely adopted PS architecture ~\cite{Dean:2012:LSD,Li14:OSDI}.
As illustrated in Fig.~\ref{fig:architecture}, this architecture includes workers, PSs, and the training dataset.
The training dataset is usually evenly divided into smaller partitions, each of which is trained by a worker.
The workers process data in parallel. % to expedite the training process of DNN.
In each iteration of the training process, each worker fetches one mini-batch of samples from its local dataset and computes a stochastic gradient.
Upon finishing computation, each worker sends the gradient to the PSs, which is subject to network %ing and communication 
 constraints (e.g., bandwidth).
In the training process, an ``epoch'' is referred to as the duration that the workers exhaust all the samples in the training dataset.

At the PS side, the received gradients from the workers are aggregated, which will in turn be used to update the model parameters following an optimization algorithm, e.g., the stochastic gradient descent (SGD) method.
Once the update is completed, the workers will pull the updated parameters from the PSs, fetch the next mini-batch of samples and proceed to the next iteration.
This process repeats until some convergence criterion of the optimization algorithm is met.

The gradient computation at each worker is based on the specific DNN  % model. , which is a deep neural network in essence. 
as illustrated in Fig.~\ref{fig:DNN}.
%a typical DNN includes the input layer, the hidden layer(s), and the output layer.
In each iteration, one mini-batch of samples is used by a worker to compute the loss from the initial layer to the last layer, which is referred to as {\em forward propagation} (FP).
After FP, a stochastic gradient of the DNN model parameters will be computed in the reverse order of layers in a {\em backward propagation} (BP) fashion.
The computed gradients are used for updates at the PSs.


%\begin{figure}[t!]
%\centering
%\begin{minipage}{.49\columnwidth}
%   \centering
%  \includegraphics[height=0.11\textheight]{Figures/fig_Distr_ML.eps}
%  \vspace{-.2in}
%  \caption{PS-based architecture.}
%  \label{fig:architecture}
%\end{minipage}%
%\hspace{0.001\columnwidth}%
%% \vspace{-0.5in}
%\begin{minipage}{.50\columnwidth}
%   \centering
%   \vspace{-0.2in}
%  \includegraphics[height=0.12\textheight]{Figures/DNN.eps}
%   \vspace{-.06in}
%  \caption{DNN training.}
%  \label{fig:DNN}
%\end{minipage}
%\vspace{-.2in}
%\end{figure}

\begin{figure}[t!]
\centering
\begin{minipage}{.23\textwidth}
   \centering
  \includegraphics[height=0.11\textheight]{Figures/fig_Distr_ML1.eps}
  \vspace{-.06in}
  \caption{PS-based architecture.}
  \label{fig:architecture}
\end{minipage}%
\hspace{0.001\columnwidth}%
\begin{minipage}{.25\textwidth}
   \centering
  \includegraphics[height=0.116\textheight]{Figures/DNN.eps}
  \vspace{-.06in}
  \caption{DNN training.}
  \label{fig:DNN}
\end{minipage}
\vspace{-.2in}
\end{figure}
\subsection{DNN Training in Distributed Computing Clusters}
To deploy DNN training jobs in a distributed computing cluster, PSs and workers are usually implemented as virtual machines or containers.
A scheduler in the computing cluster is responsible for managing the resource allocation to support the training jobs (e.g., Mesos ~\cite{Hindman11:Mesos} for a TensorFlow cluster ~\cite{TensorFlow} and Yarn ~\cite{Vavilapalli13:Yarn} for clusters running MXNet ~\cite{MXNet}).
These schedulers let users specify the resource demands (e.g., the numbers of workers and PSs, and the numbers of CPUs and GPUs), and the allocated resources usually remain unchanged throughout the training process.
%For example, in Amazon EC2, upon the submission of a training job, the user specifies his/her resource demands (e.g., the numbers of workers and PSs, the numbers of CPUs and GPUs, etc.).

Clearly, the training completion time of a job is significantly affected by resource allocation.
For example, studies in ~\cite{Peng18:Eurosys} showed that the fastest training speed was achieved when eight workers and 12 PSs were allocated to synchronously train a ResNet-50 model ~\cite{He16:ResNet50} on the ImageNet dataset ~\cite{ImageNet} (the total number of workers and PSs is fixed to 20) in their cluster.
It was also shown in ~\cite{Peng18:Eurosys} that increasing resources did not contribute to a linear increase of the training speed and could even slow down the training process.
Clearly, the fixed numbers of workers and PSs specified by users are often suboptimal.
This motivates us to design resource scheduling algorithm to determine optimal numbers of workers and PSs to achieve the fastest training speed.



==> Supporting_Preambles/jackmac.tex <==
%>From snoeyink%cs.ubc.ca@cs.Technion.AC.IL Wed Nov  3 08:18:27 1993
%Received: from csmail.cs.technion.ac.il by math.tau.ac.il (5.67/math.tau-930921)
	%id AA17625; Wed, 3 Nov 93 08:18:23 +0200
%Received: from csc (csc.cs.technion.ac.il) by csmail.cs.Technion.AC.IL (4.1/3.14)
	%id AA14244; Wed, 3 Nov 93 01:19:10 IST
%Received: from csa by csc (4.1/3.14)
	%id AA24688; Wed, 3 Nov 93 01:19:48 IST
%Received: from grolsch.cs.ubc.ca by csa (4.1/3.14)
	%id AA20525; Wed, 3 Nov 93 01:11:28 IST
%Return-Path: <snoeyink@cs.ubc.ca>
%Received: from cascade.cs.ubc.ca by grolsch.cs.ubc.ca with SMTP id AA13516
  %(5.65c/IDA-1.3.5 for alon@cs.Technion.AC.IL); Tue, 2 Nov 1993 13:56:34 -0800
%Date: Tue, 2 Nov 1993 13:56:34 -0800
%From: Jack Snoeyink <snoeyink%cs.ubc.ca@cs.Technion.AC.IL>
%Message-Id: <199311022156.AA13516@grolsch.cs.ubc.ca>
%Received: by cascade.cs.ubc.ca (4.1/SMI-4.1)
	%id AA21873; Tue, 2 Nov 93 13:56:33 PST
%To: alon@cs.Technion.AC.IL
%In-Reply-To: Alon Efrat's message of Sun, 31 Oct 93 23:38:48 IST <9310312138.AA19880@csc>
%Subject: LaTex Macros
%Status: RO
%Content-Length: 19065
%X-Lines: 638
%
%
%I'm in oberwolfach w/ micha, so I';ll just send you this and answer
%your questions on it when I get back to vancouver next week...
%
    %o                                    Jack
  %_/\_.
%(')>-(`)                          snoeyink@cs.ubc.ca
%----figbox.tex----

% 12 Oct 90 LaTeX figure boxing macros  by Jack Snoeyink
%					w/ ideas from John Hershberger
%					and code from Tom Rokicki
%%%%%%%%%%%%%%%%%
% 
% This file contains two classes of macros for dealing with figures in
% Latex documents:  
%  \figbox (and its relatives) take a box containing a figure or table
%    or whatever, caption it, and either place it on the page and wrap the
%    text around it or let it float (as usual).
%  \boxeps and \boxps take encasulated or plain postscript from a file
%    and put it in a box for use by \figbox
%
%%%%%%%%%%%%%%%%
%
% The most important macro for dealing with boxes is:
%
% \figbox: caption a box as a figure or table and place it in the margin
% 	(a marginal box) or float it (a floating box).
% 	Wide marginal boxes are promoted to one column floats; wide one
% 	column floats are promoted to two column floats.
%
% Usage: \figbox [*htblr] {box} {style} {label} {caption}
%
% The optional argument default is [htb].  Other choices
%   * two column (must come first),
%   h here, t top, b bottom (as in latex),
%   l left, r right (marginal boxes that do not float)
%
% NB: Left and right marginal boxes will not overlap in height.
%
% Two column figures default to htb unless some other 
%   	options follow the *.
%   They can also be specified by style {figure*} or {table*}.
%
% box is a box containing a figure or table.
% style is the caption style {figure}, {figure*}, {table}, or {table*}.  
% label is the label assigned.
%	if empty, the figure will not be labeled.
% caption is of the form {}, {Caption} or {[short caption] Long caption},
%       where the short caption goes into the list of figures/tables.
%	if empty, the figure will not be captioned or labeled.
% 
% The lower level macro \captionbox, described much later, can be used
% to combine two or more captioned figures into a single marginal or
% floating box.
%
%%%%%%%%%%%%%%%%
%
% options defined by macros are: \captionstyle \boxcaptionstyle
% \maxfigfraction \figboxhang \figboxmargin 
%
% \captionstyle is executed for all floating box captions
% \boxcaptionstyle is executed for all marginal box captions.
%	Default \raggedright
% \maxfigfraction is the maximum fraction of a column that can be taken up
% 	by a marginal box before it gets converted to a float.
% 	Default .6
% dimen \figboxhang is the distance a marginal box hangs into the margin.
%	Default 0pt
% dimen \figboxmargin is the width of space between the text and a
% 	marginal box. 
%	Default .15in
%
%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%
%
% The most important macros for turning postscript into boxes are:
% 
% \boxeps: Form a box containing encapsulated postscript from a file at a
%	given scale.
% \boxps: Form a box containing postscript from a file at a given scale, 
% 	width, and height.
% 
%
% Usage: \boxeps[local commands] {file} {scale}
%	 \boxps[local commands] {file} {scale} {width} {height}
%
% The optional local commands are executed after scaling. As described
% 	below, they are useful for setting origins, non-uniform scaling, etc?
% file is the filename in the \figuredirectory and without the .ps
% 	extension.
% scale is a real number: 1 to use the drawn size.  0.9 to use 90% of
% 	drawn size.  Can be changed by local commands. (see below)
% width and height are dimensions of the box produced by \boxps.
%
%%%%%%%%%%%%%%%%
%
% options: \DVIscaling \figuredirectory \missingfigure \boxer
% local commands: \horizscale \vertscale
%
% \DVIscaling is the number the dvi to ps converter considers a unit
% 	scaling transformation.  Default: 1 for dvi2ps  --- 100 for
% 	some of Rokicki's versions of dvips.
%
% \globalscaling is the scaling applied to every picture --- useful
% 	for making double size figures for journals.  Default: 1
%
% \figuredirectory is the pathname where figure postscript files are kept.
%	Default: ./figure
%
% \missingfigure{file} is executed when the file is not found.
%	Default: \def\missingfigure#1{\hbox{Missing figure #1.ps}}
%
% \boxer is the command used by \boxps to make a box of the desired size
% 	containing the figure.  Possible commands depend on the origin of
% 	the figure, and include \llboxer \lcboxer \ulboxer and \ccboxer.
% 	(ll = lower left, ul = upper left, cc = dead center, etc.)
%	\boxer can be defined in the local commands or globally.
%
% Local commands \horizscale, and \vertscale can scale the picture
% 	horizontally and vertically by different factors.  \scale
% 	scales the picture uniformly.  Scales accumulate.
%
%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%
%
% Default options
%

\def\captionstyle{}
\def\boxcaptionstyle{\raggedright}

\def\maxfigfraction{.6}% 	--- max frac of column for marg figure

\newdimen\figboxmargin%		--- margin between text and picture
\figboxmargin = .15in

\newdimen\figboxhang%		--- amount to hang picture into margin
\figboxhang = 0pt

\def\DVIscaling{1}%		--- for dvi2ps
\def\globalscaling{1}%		--- for scaling everything
\def\figuredirectory{./figures}%--- where to find the .ps files 
\let\boxer=\llboxer%		--- default origin in lower left for non-
%				      encapsulated postscript figures

\def\missingfigure#1{\hbox{Missing figure #1.ps}}


%%%%%%%%%%%%%%%%
%
% Use latex internals
%
\catcode `\@=11
\special{! /@scaleunit 1 def }

\newbox\figurebox

\def\figbox{%	[place] box style label caption
\@ifnextchar[{\figboxaux}{\figboxaux[htb]}}

%
% Parse position parameters and try appropriate placement
%
\long\def\figboxaux[#1#2]#3#4#5#6{%	--- want left margin figure?
\writepict{{#3}{#4}{#5}{#6}}%		--- save figure if journalpicts
\setbox\figurebox\hbox{#3}%
\if l#1\tryleftbox{#4}{#5}{#6}%
\else%					--- want right margin figure?
\if r#1\tryrightbox{#4}{#5}{#6}%
\else%					--- want one or two column figure?
\if *#1\checktwocoloptions#2]{\box\figurebox}{#4*}{#5}{#6}%
\else\tryonecol[#1#2]{#4}{#5}{#6}%
\fi
\fi
\fi\ignorespaces}

%
% Try a placement; promote if too wide
%

\long\def\tryleftbox#1#2#3{%		--- does left margin figure fit?
\ifdim\wd\figurebox>\maxfigfraction\columnwidth \tryonecol[htb]{#1}{#2}{#3}%
\else\leftbox{\captionbox{\box\figurebox}{#1}{#2}{#3}}\fi}

\long\def\tryrightbox#1#2#3{%	--- does right margin figure fit?
\ifdim\wd\figurebox>\maxfigfraction\columnwidth \tryonecol[htb]{#1}{#2}{#3}%
\else\rightbox{\captionbox{\box\figurebox}{#1}{#2}{#3}}\fi}

\def\checktwocoloptions{%	--- make sure twocol has htb or p
\@ifnextchar]{\floatbox[htb}{\floatbox[}}

\long\def\tryonecol[#1]#2#3#4{%	--- does one column figure fit?
\ifdim\wd\figurebox>\columnwidth \floatbox[#1]{\box\figurebox}{#2*}{#3}{#4}%
\else\floatbox[#1]{\box\figurebox}{#2}{#3}{#4}\fi}

%
% Do the work for a floating box.
%
% \floatbox[place]{box} {style} {label} {caption}
%

\long\def\floatbox[#1]#2#3#4#5{%
\begin{#3}[#1]
\hbox to \hsize{\hfil#2\hfil}
\captionandlabel{#3}{#4}{#5}
\end{#3}
}


%
% Make a caption the width of the box with given style. 
%
%\captionbox {box} {style} {label} {[optshortcap] caption}
%
% options: \boxcaptionstyle 
%
%%%%%%%%%%%%%%%%
%
% This can be used with box commands (\hbox, \vbox, \mbox, and the like),
% along with \figbox with an empty caption, to place two or more captioned
% boxes in a single marginal or floating box.   
%
% e.g. \figbox{\hbox{
%		     \captionbox{ \boxeps{fig1}1} {figure} {f1} {a figure}
%		     \hskip 1in
%		     \captionbox{ \boxeps{tab1}1} {table} {t1} {a table}
%		    }} {figure} {ignored-label} {}
%

\long\def\captionbox#1#2#3#4{% box style label {[optshortcap] caption}
\setbox\figurebox\hbox{#1}%
\parbox[t]{\wd\figurebox}{%
\bigskip\box\figurebox
\let\captionstyle=\boxcaptionstyle
\captionandlabel{#2}{#3}{#4}
\bigskip
}}

%				--- caption and label if label is nonempty
\def\captionandlabel#1#2#3{% 	--- {style} {label} {caption}
\def\testit{#3}%
\ifx\testit\empty\else%		--- if non empty caption
\writecapt{{#1}{#2}{#3}}%	--- save for journal figs
\captypeunstarred#1*.%		--- remove optional stars
\getcaption#3\endc@ption%       --- parse the caption
\def\testit{#2}%		--- check for empty label
\ifx\testit\empty\else\label{#2}\fi
\fi}

\def\captypeunstarred#1*#2.{%	--- remove two-column star from style
\def\@captype{#1}}

%
% Parse the caption of the form {caption} or {[short] long caption} 
%

\def\getcaption{\@ifnextchar[{\getcaptwo}{\getcapone}}
\long\def\getcapone#1\endc@ption{\caption[#1]%
{\def\baselinestretch{1}\Large\normalsize\captionstyle\ignorespaces #1}}
\long\def\getcaptwo[#1]#2\endc@ption{\caption[#1]%
{\def\baselinestretch{1}\Large\normalsize\captionstyle\ignorespaces #2}}

%
% Do the right thing with an already captioned marginal box
%
% \leftbox{box}
% \rightbox{box}
%
% options: \figboxmargin \figboxhang \figuredirectory

\newdimen\figboxht
\newcount\figboxn


\newcount\figboxlines%		--- picture height in number of lines
\newdimen\figboxwid%		--- picture width

\newif\ifisleftbox

\long\def\leftbox#1{%
\setbox\figurebox\hbox{#1}\global\isleftboxtrue
\startmarginbox
\vadjust{\smash{\rlap{\hskip\hsize\hskip\figboxhang
\llap{\raise.7\baselineskip\box\figurebox\hskip\rightskip}}}}%
\endmarginbox%
}

\long\def\rightbox#1{%
\setbox\figurebox\hbox{#1}\global\isleftboxfalse
\startmarginbox
\smash{\llap{\raise.7\baselineskip\box\figurebox\hskip\figboxmargin}}%
\endmarginbox%
}

\def\startmarginbox{%
\ifvmode\passpict\let\endmarginbox=\indent
\else\message{WARNING: marginbox in not in vmode}\hfilneg\ \passpict
\let\endmarginbox=\relax\fi
%
\figboxht=\dp\figurebox%	 actual height
\advance\figboxht by 1.3\baselineskip% round up
\vskip\figboxht\penalty-300\vskip-\figboxht% filbreak trick
\divide\figboxht by\baselineskip%      how many lines?
\global\figboxlines=\figboxht
%
\global\figboxwid=\wd\figurebox
\global\advance\figboxwid by \figboxmargin
\global\advance\figboxwid by -\figboxhang
\setmypar\noindent}
%

%
% Useful macros
%
% for lengthening (and shortening) picture space
%
\def\addlines#1{\global\advance\figboxlines by #1\myparshape}
\def\zerolines{\origpar\global\figboxlines=0\myparshape}

%
% for passing any marginal figures
%
\def\passpict{\par\ifnum\figboxlines>1\vskip\figboxlines\baselineskip
\zerolines\fi}

\def\emptybox#1#2{\hbox to #1{\vbox to #2{\vss}\hss}}

%%%%%%%%%%%%%%%%%%%%%
%\par hacking  
% We define our own version of Tex's \par and tell Latex it is the original

\global\let\origpar=\@@par%	--- Latex's saved version of Tex's \par
\global\let\dopar=\origpar
\global\def\@@par{\dopar}
\@setpar{\dopar}

\def\setmypar{\global\let\dopar=\mypar
\global\prevgraf=0\myparshape}

\def\mypar{\origpar\global\advance\figboxlines by -\prevgraf%
\global\prevgraf=0\myparshape}

\def\myparshape{\relax%
\ifnum\figboxlines>1\theparshape \else
\global\hangindent=0pt\global\hangafter=1%  these sometimes get restored...
\global\let\dopar=\origpar\fi}

\def\theparshape{%
\ifisleftbox\global\hangindent=-\figboxwid 
\else\global\hangindent=\figboxwid \fi
\global\hangafter=-\figboxlines \global\advance\hangafter by 1%
}


%%%%%%%%%%%%%%%%
%
%  Macros to make the list of figures and captions used by journals
%
%  To use, execute \journalpicts{scalefactor} at the beginning of the
%  file.  All figbox figures and tables will be written to a .pic file
%  and all captions to a .cap file.  On \enddocument, these files are
%  read in and the lists of figures and captions are produced.
%  
%  For non-english versions, or to add other types of floats, the
%  macro \definefnum should be changed.
%

\def\definefnum#1{%		--- ugly latex hacking to get the
%		 			right figure/table name 
\def\fnum@figure{Figure \ref{#1}}%
\def\fnum@table{Table \ref{#1}}%
\def\fnum@code{Algorithm \ref{#1}}%
}

\def\writepict#1{}
\def\writecapt#1{}

%%%%%%%%%%%%%%%%
% \journalpicts{globalscalefactor} writes all pictures and captions to
% 	files and modifies \enddocument to read these files and
% 	produce lists of enlarged figures and of captions
% 

\def\journalpicts#1{% 		global scale factor
\newwrite\pictfile
\newwrite\captfile
%
\openout\pictfile\jobname.pic
\openout\captfile\jobname.cap
%
\gdef\writepict##1{\unexpandedwrite\pictfile{\doit##1}}%
\gdef\writecapt##1{\unexpandedwrite\captfile{\doit##1}}%
%
\global\let\ENDdocument=\enddocument
\gdef\enddocument{\DOjournalpicts{#1}\ENDdocument}
}

%
%	generate enlarged figures 1 per page and list captions
%
\def\DOjournalpicts#1{{%
\def\writepict##1{}\closeout\pictfile
\def\writecapt##1{}\closeout\captfile
\@fileswfalse%			--- turn off toc, lof, and so on.
%
\onecolumn
\def\globalscaling{#1}
\def\doit##1##2##3##4{%		--- print a picture on blank page
%					{box}{style}{label}{caption}
\figboxaux[t]{\hss##1\hss}{##2}{}{}%
\vspace*{1in}
\definefnum{##3}%		--- use Figure \ref{label} or Table \ref{label}
\captionandlabel{##2}{}{##4}
\clearpage}%
%
\input\jobname.pic
%
\def\doit##1##2##3{%		--- print caption
%					{style}{label}{caption}
\definefnum{##2}%		--- use Figure \ref{label} or Table \ref{label}
\captionandlabel{##1}{}{##3}}%
%
\raggedright\let\captionstyle=\raggedright
\def\@makecaption##1##2{##1: ##2\par}%  --- Be sure captions aren't centered
%
\input\jobname.cap
}}%				--- to be followed by \enddocument



%%%%%%%%%%%%%%%%
%
%  Box macros
%
%%%%%%%%%%%%%%%%
%
% \boxeps[local commands] {file} {scale}
%
% options \DVIscaling \figuredirectory \scale \horizscale \vertscale
% \missingfigure \globalscaling
%
% \boxps[local commands] {file} {scale} {width} {height}
%
% \scale \horizscale \vertscale 

%
%  Various `boxers' --- which one is used depends on where the origin
%  of the picture is.  If you are using the bounding boxes of
%  encapsulated postscript, just use the default \llboxer.  Otherwise,
%  you have to figure out where the origin is and set \boxer appropriately.
%

\def\llboxer#1{\vbox to \figboxht{\vfil\hbox to \figboxwid{#1\hfill}}}
\def\lcboxer#1{\vbox to \figboxht{\vfil\hbox to \figboxwid{\hfill#1\hfill}}}
\def\oldboxer#1{\vbox to \figboxht{\vfil
		      \hbox to \figboxwid{\hfill\llap{#1\hskip4.25in}\hfill}}}
\def\ulboxer#1{\vbox to \figboxht{\hbox to \figboxwid{#1\hfill}\vfil}}
\def\ccboxer#1{\vbox to \figboxht{\vfil
			\hbox to \figboxwid{\hfill#1\hfill}\vfil}}

% a macro to strip the pt off a dimension
%
{\catcode`\p=12\catcode`\t=12
\gdef\removedimen#1pt{#1}}

\def\defscaled#1#2{#2=\DVIscaling#2%
\xdef#1{\expandafter\removedimen\the#2}}

\def\DVIspace{ }
\newdimen\hscalefactor
\newdimen\vscalefactor

\def\scale#1{\horizscale{#1}\vertscale{#1}}
\def\horizscale#1{\hscalefactor=#1\hscalefactor\figboxht=#1\figboxht}
\def\vertscale#1{\vscalefactor=#1\vscalefactor\figboxwid=#1\figboxwid}

%%%%%%%%%%%%%%%%
%

\def\boxps{%
\@ifnextchar[{\boxpsaux}{\boxpsaux[\relax]}}

\def\boxpsaux[#1]#2#3#4#5{%
{\figboxwid#4\figboxht#5\hscalefactor=1pt\vscalefactor=1pt%
\scale{#3}%
\scale{\globalscaling}%
#1%
\defscaled\DVIhscale\hscalefactor
\defscaled\DVIvscale\vscalefactor
\boxer{\special{psfile=\figuredirectory/#2.ps \DVIspace
		hscale=\DVIhscale\DVIspace 
		vscale=\DVIvscale}}}%
}


%%%%%%%%%%%%%%%%
% The following is from tex/inputs/epsf.tex by Tom Rokicki
% with slight modifications by Jack Snoeyink.
%
%   Written by Tomas Rokicki of Radical Eye Software, 29 Mar 1989.
%
%   Include an ecapsulated postscript graphic.
%   Works by finding the bounding box comment.
%
\newread\Epsffilein
\newif\ifEpsffileok
\newif\ifEpsfbbfound

\newdimen\pspoints
\pspoints=1in
\divide\pspoints by 72


\def\boxeps{%
\@ifnextchar[{\boxepsaux}{\boxepsaux[\relax]}}
\def\boxepsaux[#1]#2#3{%
%
%   The first thing we need to do is to open the
%   PostScript file, if possible.
%
\openin\Epsffilein=\figuredirectory/#2.ps 
\ifeof\Epsffilein\message{I couldn't open \figuredirectory/#2.ps }%
\missingfigure{#2}
\else
%
%   Okay, we got it.  Now we scan lines until we find one
%   that doesn't start with a percentage sign.  We're
%   looking for the bounding box comment.
%
   {\Epsffileoktrue\Epsfbbfoundfalse
    \catcode`\%=11 \catcode`\\=11
    \catcode`\{=11 \catcode`\}=11
    \catcode`\$=11 \catcode`\^=11
    \catcode`\&=11 \catcode`\#=11
    \catcode`\~=11 \catcode`\_=11
    \loop
       \read\Epsffilein to \Epsffileline
       \ifeof\Epsffilein\Epsffileokfalse\else
%
%   Now we check to make sure the first character is a % sign,
%   and that the rest are `%BoundingBox:' if necessary.
%
          \expandafter\Epsfaux\Epsffileline . .\\%
       \fi
   \ifEpsffileok\repeat
   \ifEpsfbbfound
	\figboxht=\Epsfury\pspoints
	\advance\figboxht by-\Epsflly\pspoints
	\figboxwid=\Epsfurx\pspoints
	\advance\figboxwid by-\Epsfllx\pspoints
   \else
	\message{No bounding box comment in \figuredirectory/#2.ps }%
	\figboxwid=2in\figboxht=1in%
   \fi%
   \immediate\closein\Epsffilein
   \hscalefactor=1pt\vscalefactor=1pt%
   \scale{#3}%
   \scale{\globalscaling}%
   #1%
%
   \defscaled\DVIhscale\hscalefactor
   \defscaled\DVIvscale\vscalefactor
%
   \hscalefactor=-\Epsfllx\hscalefactor
   \hscalefactor=1.00375\hscalefactor%	--- 72.27/72 = TeXpoints/PSpoints
   \defscaled\DVIhoffset\hscalefactor
%
   \vscalefactor=-\Epsflly\vscalefactor
   \vscalefactor=1.00375\vscalefactor%	--- 72.27/72 = TeXpoints/PSpoints
   \defscaled\DVIvoffset\vscalefactor
%
   \llboxer{\special{psfile=\figuredirectory/#2.ps \DVIspace
		hoffset=\DVIhoffset\DVIspace
		voffset=\DVIvoffset\DVIspace
                hscale=\DVIhscale\DVIspace 
                vscale=\DVIvscale}} }%
\fi
}%
%
%   We need these for comparison purposes.
%
{\catcode`\%=11 \global\let\Epsfpar=\par
\global\let\Epsfpercent=%\global\def\Epsfbblit{%BoundingBox:}}%
%
%   This is our function that checks for `%BoundingBox:' and grabs the
%   values if they are found.
%
\long\def\Epsfaux#1#2 #3\\{\relax\ifx#1\Epsfpercent
   \def\testit{#2}\ifx\testit\Epsfbblit
      \Epsfsize #3 . . . .\\%
      \global\Epsffileokfalse
      \global\Epsfbbfoundtrue
   \fi\else\ifx#1\Epsfpar\else\global\Epsffileokfalse\fi\fi}%
%
%   Here we grab the values and stuff them in the appropriate definitions.
%
\def\Epsfsize#1 #2 #3 #4 #5\\{\global\def\Epsfllx{#1}\global\def\Epsflly{#2}%
   \global\def\Epsfurx{#3}\global\def\Epsfury{#4}}%




\catcode`\@=12 			% done with with internals

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% For backward compatability
%
% \pic file; height in inches; width in inches; caption\par
% \picsc file; ht (in); wid (in); scale; caption\par
%
% \mpic file; height in inches; width in inches; caption\par
% \mpicsc file; ht (in); wid (in); scale; caption\par
%
%%%%%%%%%%%%%%%%

\def\pic#1;#2;#3;#4\par{\picsc#1;#2;#3;1;#4\par}% file; wd; ht; caption 

\def\picsc#1;#2;#3;#4;#5\par{% file; wd; ht; scale; caption
\figbox[htb]{\boxeps{#1}{#4}%{#2in}{#3in}%
}{figure}{#1}{%
% (#1: #2x#3 sc #4) % 			Uncomment for debugging
#5}}


\def\mpic#1;#2;#3;#4\par{\mpicsc#1;#2;#3;1;#4\par}% file; wd; ht; caption 

\def\mpicsc#1;#2;#3;#4;#5\par{% file; wd; ht; scale; caption
\figbox[l]{\boxeps{#1}{#4}%{#2in}{#3in}%
}{figure}{#1}{%
% (#1: #2x#3 sc #4) % 			Uncomment for debugging
#5}}




